Verifying Array Manipulating Programs with Full-Program Induction

We present a full-program induction technique for proving (a sub-class of) quantified as well as quantifier-free properties of programs manipulating arrays of parametric size N. Instead of inducting over individual loops, our technique inducts over the entire program (possibly containing multiple loops) directly via the program parameter N. Significantly, this does not require generation or use of loop-specific invariants. We have developed a prototype tool Vajra to assess the efficacy of our technique. We demonstrate the performance of Vajra vis-a-vis several state-of-the-art tools on a set of array manipulating benchmarks.

==> related.tex <==
\noindent

%Proving properties of programs that manipulate arrays of parametric size
%poses a significant  challenge for automated verification tools and techniques.
%Induction on parameter N in combination with strategies to transform the
%program as well as heuristics for quantifier instantiation are used to
%simplify the problem of assertion checking.

Amongst the related techniques, \cite{lopstr12} comes closest to ours.
They use induction on the loop counter range for verifying the given property.
%They identify recurrent fragments, which are loop bodies, such that
%one of the symbolic loop bound on the counter does not syntactically
%appear in the loop body.  The technique removes loops in the program by
%transforming them to their pre-recursive form or quantifiers by
%transforming the loops to post-recursive form.  In the pre-recursive
%representation, the loop is unrolled at the end such that the last
%iteration follows the loop wherein the upper bound is reduced by one.
%The last iteration becomes the object of analysis as the hypothesis
%generates a formula that summarizes the initial iterations.  In the
%post-recursive representation, the loop is unrolled at the beginning
%such that the first iteration is followed by the loop wherein the
%lower bound of the loop counter is increased by one.  For this form,
%the post condition is also weakened to an implication in which the
%antecedent assumes the correctness of the loop starting from the
%second iteration.  This results in a post-condition that can possibly
%be simplified to one with fewer quantifiers.  It then uses induction
%over the loop bound that appears in the given property.  For given
%pre-conditon is propagated across loops that do not update indices
%intersecting with those specified in the pre-condition.  For their
%technique to be applicable, atleast one symbolic loop bound must
%appear in the quantified property and that it must not occur in the
%loop body.  In addition, 
They require extremely restrictive data
dependency conditions, called \emph{commutativity of statements}, to
move the peel of one loop across the next sequentially composed loop
in order to get a program of the form $\PP_{N-1}; \partial{P_N}$ that
is semantically identical to $\PP_N$. Unfortunately, these
restrictions are not satisfied by a large class of programs in
practice, % (e.g. that in Fig.~\ref{fig:ex}(a) or that in
%Fig.~\ref{fig:ex}(b) with the assignment {\tt C[t3] = N;} in line 12).
making \cite{lopstr12} less useful and
%Hence the technique of~\cite{lopstr12} cannot be used to analyze these
%program.
our technique relevant.

VIAP \cite{viap} translates the program to an array-free quantified
first order logic formula in the theory of equality and uninterpreted
functions using the scheme proposed in \cite{viaptheory}.
They use several tactics to simplify the generated formula and
apply induction over array indices to prove the property.
%VIAP proved more programs than any other tool in the arrays
%sub-category in software verification competition SV-COMP 2019
%\cite{svcomp}.
Unlike our method, it does not have heuristics for finding additional
pre-conditions that are required for the induction proof to
succeed which our method successfully infers.
%Their transformation, however, is independent of the
%property to be proven unlike our technique that also
%transforms the pre- and post-conditions
%as well as uses a gaussian elimination based algorithm
%for computing weakest pre-conditions while verifying the property.


%Approaches that reason with Horn clauses have been proposed
%for proving quantified properties of array manipulating programs.
%These can be viewed as generate inductive invariants implicitly
%\cite{quic3} or explicitly \cite{madhukar19}.
QUIC3\cite{quic3} and FreqHorn\cite{madhukar19} infer universally quantified
inductive invariants of array programs specified as Constrained Horn Clauses.
\cite{quic3} extends the IC3 framework to a combination of SMT theories and
performs lazy quantifier instantiations.
\cite{madhukar19} adopts the \emph{tiling} \cite{sas17} ideas to reason with
arrays within its syntax guided synthesizes framework.
\vaphor\cite{vaphor} transforms array programs to array-free Horn formulas.
Their technique is parameterized by the number of array cells
to be tracked resulting in an eager quantifier instantiation.
%It uses Horn clause solvers such as \zthree\cite{z3}, \spacer\cite{spacer}
%and \eldarica\cite{eldarica} to verify the generated array-free Horn
%formulas.

\booster\cite{booster}
%proves quantified assertions on arrays for a class of programs.
combines acceleration \cite{acceleration1,acceleration2} and
lazy abstraction with interpolation for arrays\cite{lazyabsarray}.
Performing interpolation to infer universally quantified array
properties is difficult\cite{Jhala,Monniaux2015}.
The technique does not always succeed, especially for programs
where simple interpolants are difficult to compute\cite{sas17}.
%Among the techniques that automatically generate inductive invariants,
Template-based techniques \cite{Gulwani,Srivastava09,Dirk07}
search for invariants by instantiating the parameters of a fixed set of
templates within the abstract interpretation framework.
They can generate invariants with alternating quantifiers,
however, the user must supply invariant templates and the cost of
generating invariants is quite high.

%There are several techniques that do not require inductive invariants to be
%automatically generated.
%Fluid updates \cite{fluid} uses bracketing constraints, which are
%over- and under-approximations of indices, to specify the concrete
%elements being updated in an array without explicit partitioning.
%They assume that only a single index expression updates the array in
%each loop. Their abstraction is independent of the given property.
%

Analyses proposed in \cite{Gopan,Halbwachs} partition the
array into symbolic slices and abstracts each slice with a numeric
scalar variable.
%These techniques find it computationally difficult
%to analyze the overlap between slices and they do not handle updates
%to multiple indices in the array as well as non-contiguous array
%partitions.
%
Abstract interpretation based techniques \cite{Rival,ArrayCousotCL11}
propose an abstract domain which utilizes cell contents to split array
cells into groups.
In particular, the technique in~\cite{Rival} is useful when array
cells with similar properties are non-contiguously present in the
array.
These approaches require the implementation of abstract transformers
for each specialized domain which is not a necessity with our framework.
%

%A particular advantage of our method over the existing ones is that it enables
%use of the existing tools and techniques for reasoning over arrays, does not
%require implementation of specialized algorithms for handling quantified
%formulas and can reason with quantifiers over multiple variables.
%%
%To be able to efficiently prove wide range of problems,
%verification tools need to have an arsenal of heuristics.
%%
%Our work brings a novel program induction based heuristic to this arsenal,
%which may be adopted by these verifiers.


%--------------------- DO NOT ERASE BELOW THIS LINE --------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "aggr_main2"
%%% End: 

